Spirit Distillation: Precise Real-time Semantic Segmentation of Road Scenes with Insufficient Data

Semantic segmentation of road scenes is one of the key technologies for realizing autonomous driving scene perception, and the effectiveness of deep Convolutional Neural Networks(CNNs) for this task has been demonstrated. State-of-art CNNs for semantic segmentation suffer from excessive computations as well as large-scale training data requirement. Inspired by the ideas of Fine-tuning-based Transfer Learning (FTT) and feature-based knowledge distillation, we propose a new knowledge distillation method for cross-domain knowledge transference and efficient data-insufficient network training, named Spirit Distillation(SD), which allow the student network to mimic the teacher network to extract general features, so that a compact and accurate student network can be trained for real-time semantic segmentation of road scenes. Then, in order to further alleviate the trouble of insufficient data and improve the robustness of the student, an Enhanced Spirit Distillation (ESD) method is proposed, which commits to exploit a more comprehensive general features extraction capability by considering images from both the target and the proximity domains as input. To our knowledge, this paper is a pioneering work on the application of knowledge distillation to few-shot learning. Persuasive experiments conducted on Cityscapes semantic segmentation with the prior knowledge transferred from COCO2017 and KITTI demonstrate that our methods can train a better student network (mIOU and high-precision accuracy boost by 1.4% and 8.2% respectively, with 78.2% segmentation variance) with only 41.8% FLOPs (see Fig. 1).

==> README <==
multirow.sty  v2.8 2021/03/15
bigstruts.sty  v2.8 2021/03/15
bigdelim.sty  v2.8 2021/03/15

Original Author: Jerry Leichter
Current Author:  Pieter van Oostrum <pieter@vanoostrum.org>

 This file may be distributed under the terms of the LaTeX Project Public
 License, as described in lppl.txt in the base LaTeX distribution.
 Either version 1.3 or, at your option, any later version.

Installation:

To generate the .sty files, run the command
   tex multirow.ins
and move the resulting .sty files to a place where LaTeX can find them, preferably
..../tex/latex/multirow

Usage:

multirow.sty:

Make an entry that will span multiple rows of a table.

\multirow[vpos]{nrows}[bigstruts]{width}[vmove]{text}

vpos is the vertical positioning: t. c. or b.

nrows is the number of rows to span.  It's up to you to leave the other
      rows empty, or the stuff created by \multirow will over-write it.
      With a positive value of nrows the spanned colomns are this row and
      (nrows-1) rows below it. With a negative value of nrows they are
      this row and (1-nrows) above it.

bigstruts is mainly used if you've used bigstrut.sty.  In that case it
      is the total number of uses of \bigstrut within the rows being
      spanned.  Count 2 uses for each \bigstrut, 1 for each \bigstrut[x]
      where x is either t or b.  The default is 0.

width is the width to which the text is to be set, or * to indicate that
      the text argument's natural width is to be used.
text is the actual text.  If the width was set explicitly, the text will
      be set in a parbox of that width; you can use \\ to force linebreaks
      where you like.

      If the width was given as * the text will be set in LR mode.  If you
      want a multiline entry in this case you should use a tabular or array
      in the text parameter.

	  If the width is given as = the width will be taken from the
	  tabular column in which it appears. This only works for p{}
	  columns and similar, for example X columns in tabularx, and LCRJ
	  columns in tabulary.

      The text is centered vertically within the range spanned by nrows,
	  unless a vpos argument is given.

vmove is a length used for fine tuning:  The text will be raised (or
      lowered, if vmove is negative) by that length above (below) wherever
       it would otherwise have gone.

For example (using both multirow and bigstrut)

\newcommand{\minitab}[2][l]{\begin{tabular}{#1}#2\end{tabular}}
\begin{tabular}{|c|c|}
\hline
\multirow{4}{1in}{Common g text} & Column g2a\\
      & Column g2b \\
      & Column g2c \\
      & Column g2d \\
\hline
\multirow{3}[6]*{Common g text} & Column g2a\bigstrut\\\cline{2-2}
      & Column g2b \bigstrut\\\cline{2-2}
      & Column g2c \bigstrut\\
\hline
\multirow{4}[8]{1in}{Common g text} & Column g2a\bigstrut\\\cline{2-2}
      & Column g2b \bigstrut\\\cline{2-2}
      & Column g2c \bigstrut\\\cline{2-2}
      & Column g2d \bigstrut\\
\hline
\multirow{4}*{\minitab[c]{Common \\ g text}} & Column g2a\\
      & Column g2b \\
      & Column g2c \\
      & Column g2d \\
\hline
\end{tabular}

If any of the spanned rows are unusually large, or if you're using
bigstrut.sty and \bigstrut's are used assymetrically about the centerline of
the spanned rows, the vertical centering may not come out right.  Use the
vmove argument in this case.

Just before "text" is expanded, the \multirowsetup macro is expanded to      
set up any special environment.  Initially, \multirowsetup contains just
\raggedright.  It can be redefined with \renewcommand.
 
bigstrut.sty:

\bigstrut[pos] where pos is t or b

    Add a bit of space above, below, or both a tabular row. The amount
	is determined by \bigstrutjot.

bigdelim.sty:

\ldelim({n}{width}[text]
\rdelim){n}{width}[text]

Put a big delimiter over n rows in a tabular, optionally preceded
(\ldelim) or followed (rdelim) by text.
	

